Grasp Stability Prediction with Sim-to-Real Transfer from Tactile Sensing

Robot simulation has been an essential tool for data-driven manipulation tasks. However, most existing simulation frameworks lack either efficient and accurate models of physical interactions with tactile sensors or realistic tactile simulation. This makes the sim-to-real transfer for tactile-based manipulation tasks still challenging. In this work, we integrate simulation of robot dynamics and vision-based tactile sensors by modeling the physics of contact. This contact model uses simulated contact forces at the robot's end-effector to inform the generation of realistic tactile outputs. To eliminate the sim-to-real transfer gap, we calibrate our physics simulator of robot dynamics, contact model, and tactile optical simulator with real-world data, and then we demonstrate the effectiveness of our system on a zero-shot sim-to-real grasp stability prediction task where we achieve an average accuracy of 90.7% on various objects. Experiments reveal the potential of applying our simulation framework to more complicated manipulation tasks. We open-source our simulation framework at https://github.com/CMURoboTouch/Taxim/tree/taxim-robot.

==> text/intro.tex <==
\section{INTRODUCTION}
% robot grasping
% robot grasping with tactile
% sim2real learning

The ultimate goal of robotics is to design and build machines that can help or assist humans in a wide variety of tasks. One of the most widely used of these tasks is robotic grasping. Although this task may seem very simple for humans intuitively, it is not that easy for machines. To conduct a robust and stable grasping, the objects' external properties with respect to the robot such as location, orientation, as well as their internal properties such as mass, mass distribution, rigidity have to be considered. These properties can determine where to grasp and how to grasp, which are keys to successful grasps. Sensors from different modalities, such as vision-based, tactile-based sensors, have been used to perceive and sense the properties of objects~\cite{gao2021ObjectFolder,lee2019making}. And furthermore,  grasping policies are built based on the sensing and perception adaptively~\cite{feeling_of_sucess,pinto2016curious,more_than_a_feeling}.

The robustness and stabilization of grasping require the model to be generalized on various objects, different circumstances and. Learning-based methods provide promising solutions~\cite{joshi2020robotic,more_than_a_feeling} with the training on the large-scale dataset. However, this type of method is limited to the data acquirement and repeated experiment conduction in the real life. As a good solution to this, simulation has gained attention as it provides a realistic experiment environment and unlimited data. Several sim-to-real (sim2real) learning approaches~\cite{rao2020rl,ding2020sim} have been proposed to demonstrate the improvement of the grasp. 

With the trend of vision-based tactile sensing, different robotic manipulation tasks including the grasping task have been realized with the new generation of tactile sensors. However, due to the lack of the integrated realistic vision-based tactile simulator, the sim2real learning with vision-based tactile sensing is still under exploration. Several recent works in vision-based tactile simulation~\cite{agarwal2021simulation,tacto} have been introduced and shown the ability to reproduce the robot manipulation experiments in the simulation with high success rates. But few of them have considered the sim2real transfer and been tested on the real robot. 

\begin{figure}
    \centering
    \includegraphics[width=0.90\linewidth]{figs/teaser.jpg}
    \caption{Sim2Real grasping stability prediction.}
    \label{fig:teaser}
\end{figure}

% In this section, we conduct experiments on different objects in both simulation and real world, to evaluate the proposed framework. We aim to answer the following three research questions.
% \begin{itemize}
%     \item \textbf{RQ1}: How does our model trained in the simulator perform in the real world data? Does introducing the simulation data help in generalizing in the real world datasets?
%     \item \textbf{RQ2}: What is the effect of dataset size on model performance? Does more simulator data mean better generalization performance?
%     \item \textbf{RQ3}: What is the role of each of the physical and tactile simulations? To what extent do they have an impact on the final performance?
% \end{itemize}

Although Sim2Real research is gaining increasing popularity, there has been little progress in the field of tactile sim2real. The extent to which tactile simulation can help real world applications is still unclear. Some key research questions, such as the extent to which physical simulation and tactile simulation each play a role in the sim2real process, are still in the debate. Inspired by the above questions, we focus on building an integrated tactile simulation framework and test the performance of sim2real on the task of grasping. The experimental results show that tactile simulation has tremendous Sim2Real capabilities.

The main contributions of this work can be summarized as follows:
\begin{itemize}
    \item We introduce a new way of simulating the indentation of the grasping contact with the tactile sensors. We skilfully avoided the time-consuming and inaccurate soft-body simulation by measuring a linear relationship between the contact force and the contact volume in the real-world grasping experiments.

    \item We present an integrated simulation framework for grasping with Gelsight~\cite{gelsight} tactile sensor. We improve the optical tactile simulation performance of TACTO~\cite{tacto} with Taxim~\cite{si2021taxim}.
    % \item \st{We alleviate the sim-to-real gap by aligning all key factors in the physics simulation, such as friction and weights, based on th real world data. This alignment ensures the consistency of grasping results between the simulation and the real robot.}
    \item We conduct zero-shot learning experiments on the real world grasping datasets with the help of the proposed simulation framework. On a grasp stability prediction task, zero-shot transferring can achieve 70.8\%-100\% accuracy in real-world datasets. We show that the tactile sim2real learning can help the real-world task.
    % \item We conduct grapsing experiments on 12 objects from YCB dataset~\cite{Calli_2015} to collect data in both the simulation and the real robot. We train a grasp stability prediction model which takes tactile images as input and outputs the grasp success rate using only the simulation data. Following tests on the real-world data shows that the trained model can achieve excellent performance in the zero-shot transferring scenario. This proves the effectiveness of our proposed framework.
\end{itemize}


% Different properties can be gained from different modalities of sensing. Traditionally, vision-based methods are applied to locate and track the objects in the work space[][], and estimate the grasping poses[][] to increase the chance of success. However, vision-based methods can easily be affected by the environments, such as light conditions, the occlusion which could lead to failure of the grasping due to the poor generalization of models. Alternatively, the tactile-based grasping methods rely on the rich contact information such as slippage[][] and sensing of object's physical properties[][] from the tactile sensors and provide informative guidance of grasping. This compensate the sensitive-to-the-environment drawback of vision-based grasping methods. 

==> text/relatedwork.tex <==
\section{RELATED WORK}
\subsection{Grasping with tactile sensing}
The complexity of the grasping makes it heavily rely on the data-driven methods~\cite{data-driven-survey}. Vision data were used in ~\cite{hand-eye-grasp} for training a convolutional neural network to predict the success probability of grasping.~\cite{grasp_adaptation} proposed a grasp adaptation strategy to estimate the grasp stability by handling the uncertainties about physical propertied of objects via tactile sensing. By extending to multi-modality, ~\cite{feeling_of_sucess} showed that with the assisting of tactile data, visuo-tactile deep neural network model can improve the ability to predict the grasp. And furthermore, the author proposed an end-to-end action-conditional model to learn the regrasping policies from visual and tactile sensing in~\cite{more_than_a_feeling} ~\cite{tactile-grasp} presented a kernel-logistic-regression model to predict pose and touch-based grasp success probability. 

Dex-Net~\cite{dexnet} was presented as a dataset of 3D object models and an cloud-based algorithm for robust grasps exploration and planning. The probability of successful grasps are estimated by considering the uncertainty in object and gripper pose and friction. To increase the scale of grasping dataset and decrease the learned model's over-fitting issue,~\cite{self-suprvision} proposed a self-supervision framework for robot grasping task and show the benefits of large-scale datasets can improve the generalization of the model. Alternatively to break through the data limitation, an exploration-based grasping method with visual and tactile data was developed and tested in the simulation~\cite{Exp_Grasp_sim}. But this work didn't address the sim-to-real transfer.~\cite{mat_sim2real} proposed an end-to-end tactile grasping policy trained in the simulation and transferred to the real world with high fidelity. In our work, We also address the grasping stability estimation and regrasp planning tasks in sim2real approach but with a high-resolution tactile sensor, Gelsight which can provide rich contacting informaiton but leads to more challenge on the sim-to-real transfer.

\subsection{Physics Simulation}
The physics simulation is a complicated research and engineering problem, involving partial differential equation model and numerical calculation. In this section, we only discuss simulators that have the potential to be applied in tactile simulation. 

At this stage, it is still difficult for the physics simulation engine to achieve both accuracy and speed. On the other hand, since the real tactile sensor surface is a soft elastomer called gelpad, ideally we also need to introduce soft-body simulation. The mainstream physical simulation engines available are PyBullet~\cite{coumans2021}, Mujoco~\cite{mujoco}, TDS~\cite{TDS}, etc. Each of them has its own advantages and disadvantages and needs careful designs to make the pipeline work properly. There are three technical solutions that can be used as follows,

\noindent \textbf{Using SOTA soft-body simulation.}
The first approach is based on the most advanced flexible object simulation engines, such as PLASTICINELAB~\cite{huang2021plasticinelab}, Sofa~\cite{sofa}, etc., to model real-world dynamics. The advantage of doing so is that it can effectively model the possible lateral deformation of the gel pad during the gripping process, and make the tactile images more realistic when dealing with dynamic scenes such as slipping. The disadvantage of this is that soft-body simulation is often slower compared with pure rigid-body simulation. In addition, the soft-body simulation is highly dependent on the modeling model of flexible objects, such as the commonly used neo-Hookean solid model, but the parameters of these models are often very difficult to obtain in the real world.

\noindent \textbf{Using mature rigid-body simulation and partially prepared soft-body simulation.}
The second approach is based on some mature physics simulation engines, such as PyBullet~\cite{coumans2021}, which have partially supported soft-body simulation. This has the advantage of being faster and having sufficient accuracy guarantees in the dynamics of rigid objects. The problem with this, however, is that traditional physics simulation engines tend to have poor performance in soft-body simulation. In the course of our experiments, this can lead to serious numerical problems and even collapse of the whole simulation calculation.

\noindent \textbf{Using mature rigid-body simulation and experiment data fitting.}
The last one is completely based on the mature rigid body physics simulation, for which the deformation of the tactile sensor surface can be handled in the subsequent Physics-to-Tactile stage by means of experimental measurements and fitting~\cite{tacto}. This has the advantage of being fast and numerically stable since it does not require any soft-body simulation. The processing of the deformation at the contact point is performed directly inside the renderer, ensuring the accuracy of the contact surface while being very efficient. The contact area is calculated using the experimental data as a reference, and thus the generalization performance is directly guaranteed during the Sim-to-Real process.


\subsection{Simulation of Tactile Sensors and Sim2Real Learning}
Tactile sensors~\cite{tactile-review} have evolved into different generations and types and played an important part in the robotics manipulation tasks in last few decades. As a popular branch, soft optical tactile sensors with high spacial resolution have gained more attentions in the recent years, such as Gelsight~\cite{gelsight}, DIGIT~\cite{digit}, soft-bubble~\cite{soft-bubble} etc. Along with the tactile sensors' roles and learning methods' domination in the robotics, an increasing number of research are studying the simulation of soft optical tactile sensors due to its capabilities and efficiency in data-collection and model prototyping. TACTO~\cite{tacto} was the first work to integrate vision-based tactile sensors into an physics simulation framework PyBullet, which is fast, flexible and open-source. ~\cite{phong_sim} presented a realistic Gelsight tactile simulation and showed its ability for sim2real transfer learning on shape classification. ~\cite{sim2real_RL} proposed a simulation method of contact geometry as depth images and demonstrated the zero-shot sim2real policy transfer on several reinforcement learning tasks. Instead of focusing on the realistic optical signal simulation, there are also simulation work studying the contact with physics models. ~\cite{biotac} utilized the physics-based simulator to simulate the soft body deformation of interaction, and then built the generative network to project the surface's deformation to electrical signals. ~\cite{contact_force_sim} reconstructed the distribution of contact forces applied on the soft surface of tactile sensor with a learning model.

Most of the work demonstrated the good performances of various tasks in the simulators. However when narrowing down to the sim2real learning transfer, only~\cite{sim2real_RL} had comprehensive experiments that evaluated the trained models on the real robot. And none of them has worked on the grasping task which will be addressed in this paper. Grasping simulation requires not only the realistic tactile simulation but the considering of the physics of the contacting, which makes it harder than the tasks conducted in the existing work.

